Breaking Down Power Barriers in On-Device Streaming ASR: Insights and Solutions

Power consumption plays a crucial role in on-device streaming speech recognition, significantly influencing the user experience. This study explores how the configuration of weight parameters in speech recognition models affects their overall energy efficiency. We found that the influence of these parameters on power consumption varies depending on factors such as invocation frequency and memory allocation. Leveraging these insights, we propose design principles that enhance on-device speech recognition models by reducing power consumption with minimal impact on accuracy. Our approach, which adjusts model components based on their specific energy sensitivities, achieves up to 47% lower energy usage while preserving comparable model accuracy and improving real-time performance compared to leading methods.

==> limitations.tex <==
\section{Limitations\label{sec:limitation}}
The operational dynamics and memory placement of model components significantly influence the energy consumption of numerous machine learning models. Given constraints on time and computational resources, our research focuses exclusively on on-device streaming speech recognition. However, we posit that the insights and guidelines for energy efficiency optimization presented in this study could be relevant to other speech and NLP models, including, but not limited to, T5~\cite{T5} and BART~\cite{BART} (where the encoder and decoder have different invocation frequencies due to autoregressive decoding and thus have different power sensitivities). The applicability of these guidelines to other models remains an area for future investigation.
